Designing and Implementing a Generator Framework for a SIMD Abstraction Library

The Single Instruction Multiple Data (SIMD) parallel paradigm is a well-established and heavily-used hardware-driven technique to increase the single-thread performance in different system domains such as database or machine learning. Depending on the hardware vendor and the specific processor generation/version, SIMD capabilities come in different flavors concerning the register size and the supported SIMD instructions. Due to this heterogeneity and the lack of standardized calling conventions, building high-performance and portable systems is a challenging task. To address this challenge, academia and industry have invested a remarkable effort into creating SIMD abstraction libraries that provide unified access to different SIMD hardware capabilities. However, those one-size-fits-all library approaches are inherently complex, which hampers maintainability and extensibility. Furthermore, they assume similar SIMD hardware designs, which may be invalidated through ARM SVE's emergence. Additionally, while existing SIMD abstraction libraries do a great job of hiding away the specifics of the underlying hardware, their lack of expressiveness impedes crucial algorithm design decisions for system developers. To overcome these limitations, we present TSLGen, a novel end-to-end framework approach for generating an SIMD abstraction library in this paper. We have implemented our TSLGen framework and used our generated Template SIMD Library (TSL) to program various system components from different domains. As we will show, the programming effort is comparable to existing libraries, and we achieve the same performance results. However, our framework is easy to maintain and to extend, which simultaneously supports disruptive changes to the interface by design and exposes valuable insights for assessing provided functionality.

==> 01_introduction.tex <==
\section{Introduction}
\label{sec:Introduction}

%simd: nicht immer ratsam alles zu vektorisieren mit einer extension (mikhail zitieren) -> besonders im MIMD fall, wenn viele threads laufen macht es sinn teile des codes mit geringeren vektorbreite zu betreiben um zb. downscaling zu vermeiden. 
%das stellt developer vor die herausforderung denselben Algortihmus für verschiedene Vektorbreiten nicht nur zu programmieren sondern auch zu maintainen. 
%Besonders für Intel-Plattformen stellt das eine Herausforderung dar, da die verschiedenen SIMD-Extensions (SSE, AVX, AVX512) sich nicht nur in den verfügbaren Vektorbreiten sondern auch im Funktionsumfang teils drastisch unterscheiden.
%
%Eine notable recent Entwicklung ist die FPGA-Accelerator Card Stratix 10 von Intel, welche über PCIe angeschlossen über USM direkt auf Host-Memory zugreifen und verarbeiten kann. 
%Die Stratix 10 kann den Memory-Bus saturieren, wenn pro Takt 64-byte geladen werden. Suprisingly, entspricht das einer SIMD-Registerbreite von 512-bit - somit lässt sich auf der Stratix 10 simdifizierter Code ausführen.
%Um dies zu erreichen muss skalarer Code annotiert werden um vom eigenen dpc++ Compiler als auf SIMD-registern operierenden Code zu erkennen. 
%-->BACKGROUND ?
%For instance, in a heavy load scenario with all existing cores active, the largest available SIMD-register size of 512 bit on Intel platforms may lead to downscaling cores, eventually harming overall performance. 
%To circumvent such behavior, some threads processing an algorithm must use smaller SIMD registers to attain optimal performance. 

\emph{Single Instruction Multiple Data (SIMD)} is a well-established parallelism concept that is characterized by the fact that the \emph{same operation} is simultaneously applied on \emph{multiple data elements} within a single instruction~\cite{DBLP:series/synthesis/2015Hughes}. 
This parallelism concept plays a crucial role in increasing the single-thread performance in data-centric as well as compute-heavy domains such as Database Systems (DB)~\cite{DBLP:conf/sigmod/PolychroniouRR15,DBLP:journals/vldb/PolychroniouR20,DBLP:conf/systor/ZarubinDKHL21}, Machine Learning Systems (ML)~\cite{DBLP:conf/icdm/BohmP15,DBLP:conf/iscc/CarneiroSN21,DBLP:journals/eaai/DiasAM04} or High-Performance Computing (HPC)~\cite{DBLP:conf/sc/ChhuganiKSPDSS12,DBLP:journals/concurrency/0001FLM21,DBLP:journals/superfri/KomatsuOFFIMSK21}. 
Modern CPUs provide evolving support for SIMD capabilities using vendor-specific SIMD instruction set extensions (SISE). 
Those extensions usually include arithmetic and Boolean operators, logical and arithmetic shifts, and data type conversions, including specific SIMD instructions to load data from main memory into SIMD registers and write it back. 
SIMD instructions can be used directly within ordinary code as they operate within the same address space as regular scalar instructions. 

Another technique to further increase the performance of data-centric and compute-heavy applications relies on the efficient use of accessible hardware like multi-cores, using (i) the \emph{Multiple Instruction Multiple Data (MIMD)} parallelism concept or (ii) ship parts of the computation to accelerator cards, e.g., graphics cards or even FPGA's. 
In contrast to SIMD, MIMD is a parallelism concept, where \emph{different operations} are executed on \emph{different data} in parallel.

Recent research investigated the opportunities and challenges of combining SIMD and MIMD for data-centric applications. 
As \cite{DBLP:conf/systor/ZarubinDKHL21} showed, such an amalgamation is only sometimes straightforward but often relies on carefully selecting the used instructions and degree of data parallelism throughout the system. 
Besides choosing the right degree of data-level parallelism per thread, this observation introduces another crucial challenge for developing and maintaining complex software systems since the same algorithm has to be implemented multiple times for different degrees of data parallelism. 
Furthermore, the available hardware landscape is becoming more and more diverse. 
As described in~\cite{TVLPaper}, SIMD capabilities can be categorized along three dimensions: (i) the size of the provided SIMD registers - or in other words, the degree of available data parallelism, (ii) the number of SIMD instructions, and (iii) the granularity of the supported bit-level parallelism, i.e., on which data widths the SIMD instructions are executable. 
For example, Intel provides SISE with SIMD registers of a size up to 512-bit (e.g., AVX-512~\cite{avx512}), while ARM processors with SIMD registers of a size of 128-bit (NEON SISE~\cite{neon}) up to 2048-bit (SVE~\cite{ARMSVE}) are on the rise. 
Moreover, the †~\cite{TVLPaper}, and there is no uniform naming convention for SIMD instructions. 

With the advent of \emph{unified shared memory (USM)}, accelerators like GPUs and even FPGAs, e.g., Intel Stratix 10, can execute and accelerate compute-heavy algorithms. 
Interestingly, FPGAs like the Stratix 10 saturate the PCIe bus when loading and processing 64-byte, or 512-bit, of data per cycle. 
Consequently, data-parallel processing becomes a critical factor in utilizing such accelerators to their maximum extent. 
Traditionally, FPGA programming relied on writing RTL code; with icpx, Intel introduced a new compiler that can compile annotated C/C++ code to an integrated circuit. 
This capability allows the integration of accelerator-specific code into CPU-targeted code. 
This development opens up a tremendous potential for further optimization of compute-heavy tasks. 
However, the challenges mentioned before stay the same -- there is no unified programming model, and developers must adapt their code for every possible hardware. 


\begin{figure}
    \begin{minipage}[t]{.40\linewidth}
        \centering 
        \small (a) Intel SSE implementation\\
        %\lstinputlisting[frame=off,language=C++]{#2}
        \inputminted[fontsize=\scriptsize,linenos=no]{cpp}{supplementary/cmpeq_sse.cpp}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.40\linewidth}
        \centering \small (b) ARM Neon implementation\\
        %\lstinputlisting[frame=off,language=C++]{#4}
        \inputminted[fontsize=\scriptsize,linenos=no]{cpp}{supplementary/cmpeq_neon.cpp}
    \end{minipage}
    \caption{Example listing for a SIMD register comparison using Intel's SSE and ARM's NEON producing an integral mask. The \emph{simdified} comparison operator of both extensions produces a SIMD register, where all bits are set to 1 within a lane if the corresponding input lanes are equal. Otherwise, all bits are set to 0. This SIMD register is used to form a mask, where a 1-bit at the n-th position indicates that the n-th values from the input registers were binary identical.}
    \label{lst:cmpeq_sse_neon}
\end{figure}


\textbf{Our Contribution and Outline:}
In general, utilizing vendor-specific SIMD intrinsics to their full extent implies a steep learning curve and a substantial manual effort for implementing and porting system components. 
Consequently, industry and research have invested considerable effort and time into designing and developing SIMD abstraction libraries to first and foremost address the portability challenge of highly optimized SIMD code.
Examples are -- making no claim to be exhaustive -- XSIMD~\cite{xsimd}, Google Highway~\cite{highway},  TVL~\cite{TVLPaper}, or the Generic SIMD Library~\cite{DBLP:conf/ppopp/WangWTSM14}.  
Those libraries are usually implemented in C/C++ for performance reasons, and they provide C++ class templates to represent a SIMD hardware register. 
The template parameter is a placeholder for the underlying type, which will reside in the register. 
Template-dependent overloaded operators or non-class function templates wrap the actual SIMD intrinsics in a type-safe manner. 
Furthermore, the templates enable compile-time deduction and code generation with zero overhead for the runtime. 
On the one hand, the manual effort for writing, maintaining, extending, and porting SIMD-aware system components decreases significantly by using those libraries. 
However, on the other hand, all existing SIMD abstraction libraries must be maintained and extended to continuously include evolving SIMD innovations, which entails tricky challenges from a library-design perspective. 
In particular, to overcome the non-negligible manual effort, we present our novel framework called \emph{TSLGen} for generating a SIMD abstraction library in this paper.
Based on that, this paper makes the following contributions: 
\begin{compactenum}
\item In Section~\ref{sec:Background}, we present related work in the context of SIMD abstraction libraries in more detail. In particular, we introduce requirements for such libraries and discuss the manual approach of existing libraries to these requirements.
\item Afterwards, we introduce our novel developed framework \emph{TSLGen} in Section~\ref{sec:TSLGen}. We start with a schematic overview before describing the individual components of our framework in more detail. As we will show, our overall approach is based on the complete generation of a SIMD abstraction library.
This makes the library much easier to maintain and extend. 
\item In Section~\ref{sec:Evaluation}, we present selective evaluation results based on use cases from different perspectives\footnote{The implementation of our \emph{TSLGen} framework, including several use-case implementations, will be made available in case of acceptance.}. In particular, we show that we can seamlessly integrate Intel FPGA cards as flexible SIMD processing units in addition to classical SIMD CPU extensions. 
\end{compactenum}
Finally, we discuss related work in a broader context in Section~\ref{sec:RelatedWork} and close the paper with a summary in Section~\ref{sec:Conclusion}.

%is available online at: \url{https://github.com/db-tu-dresden/TVLGen}.




==> 01_introduction_v2.tex <==
\section{Introduction}
\label{sec:Introduction}

%simd: nicht immer ratsam alles zu vektorisieren mit einer extension (mikhail zitieren) -> besonders im MIMD fall, wenn viele threads laufen macht es sinn teile des codes mit geringeren vektorbreite zu betreiben um zb. downscaling zu vermeiden. 
%das stellt developer vor die herausforderung denselben Algortihmus für verschiedene Vektorbreiten nicht nur zu programmieren sondern auch zu maintainen. 
%Besonders für Intel-Plattformen stellt das eine Herausforderung dar, da die verschiedenen SIMD-Extensions (SSE, AVX, AVX512) sich nicht nur in den verfügbaren Vektorbreiten sondern auch im Funktionsumfang teils drastisch unterscheiden.
%
%Eine notable recent Entwicklung ist die FPGA-Accelerator Card Stratix 10 von Intel, welche über PCIe angeschlossen über USM direkt auf Host-Memory zugreifen und verarbeiten kann. 
%Die Stratix 10 kann den Memory-Bus saturieren, wenn pro Takt 64-byte geladen werden. Suprisingly, entspricht das einer SIMD-Registerbreite von 512-bit - somit lässt sich auf der Stratix 10 simdifizierter Code ausführen.
%Um dies zu erreichen muss skalarer Code annotiert werden um vom eigenen dpc++ Compiler als auf SIMD-registern operierenden Code zu erkennen. 
%-->BACKGROUND ?
%For instance, in a heavy load scenario with all existing cores active, the largest available SIMD-register size of 512 bit on Intel platforms may lead to downscaling cores, eventually harming overall performance. 
%To circumvent such behavior, some threads processing an algorithm must use smaller SIMD registers to attain optimal performance. 

\emph{Single Instruction Multiple Data (SIMD)} is a well-established parallelism concept that is characterized by the fact that the \emph{same operation} is simultaneously applied on \emph{multiple data elements} within a single instruction~\cite{DBLP:series/synthesis/2015Hughes}. 
This state-of-the-art concept plays a crucial role in increasing the single-thread performance in data-centric as well as compute-heavy domains such as Database Systems (DB)~\cite{DBLP:conf/sigmod/PolychroniouRR15,DBLP:journals/vldb/PolychroniouR20,DBLP:conf/systor/ZarubinDKHL21}, Machine Learning Systems (ML)~\cite{DBLP:conf/icdm/BohmP15,DBLP:conf/iscc/CarneiroSN21,DBLP:journals/eaai/DiasAM04} or High-Performance Computing (HPC)~\cite{DBLP:conf/sc/ChhuganiKSPDSS12,DBLP:journals/concurrency/0001FLM21,DBLP:journals/superfri/KomatsuOFFIMSK21}. 
Modern CPUs provide evolving support for SIMD capabilities using vendor-specific SIMD instruction set extensions (SISE). 
Those extensions usually include arithmetic and Boolean operators, logical and arithmetic shifts, and data type conversions, including specific SIMD instructions to load data from main memory into SIMD registers and write it back. 
%SIMD instructions can be used directly within ordinary code as they operate within the same address space as regular scalar instructions. 
Furthermore, the availability of SIMD instructions for a particular functionality or data type varies depending on ARM, Intel, and other vendors.
This leads to a highly heterogeneous SIMD environment.

A further technique to increase the performance of data-centric and compute-heavy applications relies on the efficient use of accessible hardware such as (i) multi-cores using the \emph{Multiple Instruction Multiple Data (MIMD)} parallelism concept or (ii) shipping parts of the computation to accelerator cards, e.g., graphics cards or even FPGA's. 
However, the combined usage of SIMD and MIMD or accelerator cards provides additional challenges. 
For example,~\cite{DBLP:conf/systor/GottschlagBB20,DBLP:conf/systor/ZarubinDKHL21} showed that using only a single fixed SIMD extension, e.g., Intel's AVX512, does not yield optimal performance. 
In particular, the best-performing SISE variant depends on the level of MIMD concurrency, the memory type, and the access pattern of the application~\cite{DBLP:conf/systor/ZarubinDKHL21}. 
However, achieving the best interplay between SIMD and MIMD requires the application to be implemented for each SISE, which is an enormous effort. 
The same applies to accelerator cards, where a separate code base has to be built and maintained alongside a complex CPU variant with a SIMD-MIMD interplay. 

%Another technique to further increase the performance of data-centric and compute-heavy applications relies on the efficient use of accessible hardware like multi-cores, using (i) the \emph{Multiple Instruction Multiple Data (MIMD)} parallelism concept or (ii) ship parts of the computation to accelerator cards, e.g., graphics cards or even FPGA's. 


%Recent research investigated the opportunities and challenges of combining SIMD and MIMD for data-centric applications. 
%As \cite{DBLP:conf/systor/ZarubinDKHL21} showed, that using only one fixed SIMD extension, e.g. Intel's AVX2, does not yield optimal results.
%Moreover it is important to carefully select the best fitting extension for the parts of the algorithm, depending on data placement or system load among others.
%However, switching between different SIMD SISEs implies the availability of all the required functionality in all required SISEs, e.g. gather-scatter operations for 32 bit signed integers or a horizontal-add on registers with a width of 128, 256 and 512 bit.
%If the required functionality is not present, workarounds have to be found and incorporated in the different algorithm specifications.

To tackle some of these challenges, industry and research have invested considerable effort and time into designing and developing SIMD abstraction libraries to first and foremost address the portability challenge of highly optimized SIMD code.
Examples are -- making no claim to be exhaustive -- XSIMD~\cite{xsimd}, Google Highway~\cite{highway},  TVL~\cite{TVLPaper}, or the Generic SIMD Library~\cite{DBLP:conf/ppopp/WangWTSM14}.
Those libraries are usually implemented in C/C++ for performance reasons, and they leverage C++ class templates to represent a SIMD hardware register.
All of them have in common that they hide the concrete implementation (or workaround) behind a dedicated function call and furthermore, the templates enable compile-time deduction and code generation with zero overhead for the runtime.
Leveraging such libraries already allows writing easily exchangeable code to execute the same algorithm with different SIMD SISEs.

%In general, utilizing vendor-specific SIMD intrinsics to their full extent implies a steep learning curve and a substantial manual effort for implementing and porting system components.
%Consequently, industry and research have invested considerable effort and time into designing and developing SIMD abstraction libraries to first and foremost address the portability challenge of highly optimized SIMD code.
%Examples are -- making no claim to be exhaustive -- XSIMD~\cite{xsimd}, Google Highway~\cite{highway},  TVL~\cite{TVLPaper}, or the Generic SIMD Library~\cite{DBLP:conf/ppopp/WangWTSM14}.
%Those libraries are usually implemented in C/C++ for performance reasons, and they leverage C++ class templates to represent a SIMD hardware register.
%All of them have in common, that they hide the concrete implementation (or workaround) behind a dedicated function call and furthermore, the templates enable compile-time deduction and code generation with zero overhead for the runtime.
%Leveraging such libraries already allows us to write easily exchangeable code to execute the same algorithm with different SIMD SISEs.

\textbf{Our Contribution and Outline:}
However, building, maintaining and extending an SIMD abstraction library is non-trivial and requires, e.g. carefully placed \#\textsc{ifdef} statements to ensure seamless portability between platforms.
Adding new functionality or revising past design decisions can often incur a high refactoring effort.
To overcome that laborious manual programming part, we present our novel framework called \emph{TSLGen} for generating a SIMD abstraction library in this paper.
Based on that, this paper makes the following contributions: 
\begin{compactenum}
\item In Section~\ref{sec:Background}, we present related work in the context of SIMD abstraction libraries in more detail. In particular, we introduce requirements for such libraries and discuss the manual approach of existing libraries to these requirements.
\item Afterwards, we introduce our novel developed framework \emph{TSLGen} in Section~\ref{sec:TSLGen}. We start with a schematic overview before describing the individual components of our framework in more detail. As we will show, our overall approach is based on the complete generation of a SIMD abstraction library.
This makes the library much easier to maintain and extend and it even allows for chery picking of only a few specific parts to be generated. Thus we can either generate the complete library or only a slim library on a per use-case basis, whenever necessary.
\item In Section~\ref{sec:Evaluation}, we present selected evaluation results based on use cases from different perspectives\footnote{The implementation of our \emph{TSLGen} framework, including several use-case implementations, will be made available in case of acceptance.}. In particular, we show that we can seamlessly integrate Intel FPGA acclerator cards as flexible SIMD processing units in addition to classical SIMD CPU extensions. 
This facilitates the usage of such accelerator cards, since no specific code base needs to be implemented anymore.  
From our point of view, this is a big step forward to execute efficient arbitrary CPU-SIMD code on FPGA.  
\end{compactenum}
Finally, we discuss related work in a broader context in Section~\ref{sec:RelatedWork} and close the paper with a summary in Section~\ref{sec:Conclusion}.

%is available online at: \url{https://github.com/db-tu-dresden/TVLGen}.

